Decentralized Credential Status Management: A Paradigm Shift in Digital Trust

Public key infrastructures are essential for Internet security, ensuring robust certificate management and revocation mechanisms. The transition from centralized to decentralized systems presents challenges such as trust distribution and privacy-preserving credential management. The transition from centralized to decentralized systems is motivated by addressing the single points of failure inherent in centralized systems and leveraging decentralized technologies' transparency and resilience. This paper explores the evolution of certificate status management from centralized to decentralized frameworks, focusing on blockchain technology and advanced cryptography. We provide a taxonomy of the challenges of centralized systems and discuss opportunities provided by existing decentralized technologies. Our findings reveal that, although blockchain technologies enhance security and trust distribution, they represent a bottleneck for parallel computation and face inefficiencies in cryptographic computations. For this reason, we propose a framework of decentralized technology components that addresses such shortcomings to advance the paradigm shift toward decentralized credential status management.

==> reviewer-changes.tex <==
\section{Summary of Changes Based on Reviewers’ Feedback - Will be removed for the final version
}

Reviewer Feedback: The discussion on legal and regulatory challenges is superficial.

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Expanded discussion on legal and regulatory challenges, including compliance with GDPR, cross-border data transfer regulations, and the legal recognition of blockchain-based identities.
    \item Position: Added to the Organizational Considerations section.
\end{itemize}

Reviewer Feedback: There is a lack of practical implementation examples that demonstrate the proposed framework’s effectiveness in real-world scenarios.

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Added detailed case studies from sectors such as healthcare and education to illustrate the practical application and benefits of the proposed framework.
    \item Position: Added to the Practical Implementation Examples section.
\end{itemize}

Reviewer Feedback: How does your framework address the privacy concerns associated with publicly linking identities and public keys, which Certcoin does not adequately solve?

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Detailed how the advanced cryptographic techniques ZKP and MPC are employed to enhance privacy.
    \item Position: Added to the Related Work section, after discussing Certcoin.
\end{itemize}

Reviewer Feedback: How does your proposed framework integrate advanced cryptographic techniques like MPC and FHE to further improve privacy compared to PB-PKI?

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Elaborated on the specific use cases of MPC and FHE within the proposed framework.
    \item Position: Added to the Framework for Dynamic and Decentralized Credential Status Management section, under the subsection on cryptographic techniques.
\end{itemize}

Reviewer Feedback: In what ways does your framework incorporate SSI concepts: Artificially Intelligent Electronic Money, doi: 10.1109/MCE.2020.3024512, to provide a more user-centric and privacy-preserving identity management solution compared to CertLedger?

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Explained how SSI principles are integrated into the framework to enhance user control and privacy.
    \item Position: Added to the Identity Management subsection of the Framework for Dynamic and Decentralized Credential Status Management section.
\end{itemize}

Reviewer Feedback: How does your framework specifically integrate SSI principles with DPKI to enhance user control and privacy?

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Discussed the integration of SSI principles, including decentralized identifiers (DIDs) and verifiable credentials (VCs), to enhance user control over digital identities.
    \item Position: Added to the Identity Management subsection of the Framework for Dynamic and Decentralized Credential Status Management section.
\end{itemize}

Reviewer Feedback: What specific strategies does your framework employ to address the scalability and performance challenges identified in this analysis?

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Detailed strategies such as sharding and Layer 2 solutions to enhance scalability and performance.
    \item Position: Added to the Discussion section, under the subsection on scalability and performance.
\end{itemize}

Reviewer Feedback: The work did not well define the concept of Trust/Digital Trust/Decentralized Trust. Actually, there are some existing surveys on this topic, e.g., Surveying Trust-based Collaborative Intrusion Detection: State-of-the-Art, Challenges and Future Directions. IEEE Communications Surveys and Tutorials, vol. 24, no. 1, pp. 280-305, IEEE, 2022.

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Enhanced the definition of trust, digital trust, and decentralized trust, incorporating references to existing surveys.
    \item Position: Added to the Introduction section.
\end{itemize}

Reviewer Feedback: The related work section is not well organized, missed many references, it is because the scope is not well defined.

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Reorganized the related work section to clearly define its scope and include comprehensive references.
    \item Position: Added to the beginning of the Related Work section.
\end{itemize}

Reviewer Feedback: It lacks deep discussions on the sub-topics

Modifications and Incorporation of the Feedback:
\begin{itemize}
    \item Included Feedback: Deepened the discussions on sub-topics like cryptographic primitives, trust mechanisms, privacy considerations, and scalability challenges.
    \item Specifically enhanced the sections on MPC, FHE, ZKP, and ECC.
    \item Position: Expanded throughout the “Framework for Dynamic and Decentralized Credential Status Management” section.
\end{itemize}

==> working_folder/authors.tex <==
Patrick, Tom, Mauro


==> working_folder/dissertation_content_intro_pki.tex <==
\section{Introduction (1-2 pages)}
\label{sec:introduction}
% CSF'24 solicits systematization of knowledge (SoK) papers in foundational security and privacy research. These papers systematize, re-formulate, or evaluate existing work in one established and significant research topic. Such papers must provide new insights. Survey papers without new insights are not appropriate. Papers trying to identify robust foundations of research areas still lacking them are particularly welcome. Submissions will be distinguished by the prefix “SoK:” in the title and a checkbox on the submission form.

Digital certificates are essential to secure web communications, particularly within the HTTPS infrastructure~\cite{10.1145/3319535.3363192}. These certificates, predominantly X.509, are issued by Certificate Authorities (CAs) to authenticate domain owners, thereby enabling Transport Layer Security (TLS) connections essential for safeguarding web interactions~\cite{leavitt2011internet},~\cite{roberts2019you}. In this centralized model, CAs bear the dual responsibility of verifying the identity of requesters and establishing domain credibility, centralizing trust and control~\cite{chadwick2003role},~\cite{ saint2011representation}. While foundational for web security, centralization introduces vulnerabilities and challenges, underscoring the need for an in-depth examination of these systems' robustness and potential alternatives~\cite{birge2018bamboozling},~\cite{10.1145/2975591},~\cite{schwittmann2019domain},~\cite{adrian2015imperfect}. Centralized trust models in Public Key Infrastructure (PKI), especially those relying on X.509 certificates, confront significant challenges~\cite{10196098},~\cite{clark2013sok},~\cite{delignat2016cinderella}. Centralized architectures face security risks, notably the vulnerability of Certificate Authorities (CAs), requiring the revocation of compromised certificates~\cite{Berkowsky2017SecurityIW}.

Certificate revocation was primarily managed through Certificate Revocation Lists (CRLs) and remains a dominant methodology~\cite{10.1145/2815675.2815685}. However, revocation lists encountered scalability challenges due to the exponential increase in the volume of revoked certificates. To mitigate the constraints posed by CRLs, the Online Certificate Status Protocol (OCSP) evolved~\cite{santesson2013x}. Although the OCSP introduced real-time verification, it increased the communication overhead required for certificate status verification, imposing additional operational demands~\cite{munoz2002evaluation},~\cite{zhu2016measuring}. Despite the introduction of OCSP Must-Staple~\cite{chung2018web} and short-lived certificates~\cite{topalovic2012towards}, challenges such as irregular browser adoption still persist~\cite{8835212}. These challenges require reevaluating the management of the certificate status in the transition to decentralized systems~\cite{8406563}. The need to transition towards decentralized systems is emphasized by incidents of compromised CAs and issuance of fraudulent certificates, highlighting the vulnerability of centralized systems to security breaches. Durumeric et al.~\cite {durumeric2013analysis} analyze the HTTPS ecosystem and emphasize the fragility of centralized PKI, where a single point of failure can compromise web security globally. 

The shift from centralized to decentralized systems marks a change in digital identity verification, addressing the limitations of centralized models~\cite{Fromknecht2014ADP},~\cite{Avellaneda2019DecentralizedIW}. Central to this shift is blockchain technology, which introduces novel methodologies for managing identities and credentials~\cite{Lux2020DistributedLedgerbasedAW},~\cite{Sedlmeir2021DigitalIA}. At the heart of decentralized identity systems is the Self-Sovereign Identity (SSI) paradigm, emphasizing verifiable credentials and granting individuals direct control over their digital identities. Verifiable credentials represent a departure from traditional certificates in centralized systems~\cite{preukschat2021self},~\cite{allen2016path}. Blockchain's immutable ledger and consensus mechanisms underpin decentralized systems, ensuring cryptographic security and independently verifiable credentials without centralized authority reliance~\cite{muhle2018survey}.

The research question of this Systematization of Knowledge paper is: 
\begin{quote}
\textit{``In what ways do decentralized approaches to credential status management surpass traditional PKI methods to improve web security, user privacy, and ensure scalability and real-time verification of digital certificates?''}
\end{quote}

% TODO what are PKI methods? 
This paper differentiates itself from existing research by contextualizing traditional PKI components and methods alongside decentralized approaches. It provides a comparative analysis of decentralized methodologies such as zero-knowledge proofs and multi-party computation. Additionally, it provides a comprehensive overview of domain-specific requirements within decentralized environments for managing credential status, underscoring the unique challenges and opportunities that Decentralized Credential Status Management (DCSM) systems present. 

The evolution from traditional certificate management towards DCSM aims to provide a scalable framework for credential management, prioritizing user-centric governance in decentralized, and digital transactions. We have identified the following requirements for DCSM as essential to adapt to evolving decentralized environments. These requirements are imperative to successfully transition to a decentralized framework, ensuring that credential management is scalable, reliable, and aligned with the increasing focus on user-centric control and privacy within decentralized interactions.

\begin{enumerate}
    \item[\textbf{(R1)}] Privacy and Untraceability. The system must ensure that unauthorized entities cannot trace user identity and activities. It should employ anonymization and privacy-enhancing technologies to preserve user confidentiality.
    \item[\textbf{(R2)}] User-Centric Control. The system must prioritize user control, allowing individuals to autonomously manage their digital identities autonomously, thus increasing user autonomy and oversight. 
    \item[\textbf{(R3)}] Real-Time Revocation Mechanisms. The system must enable efficient revocation processes, allowing immediate responses to security breaches or when credentials become invalid. This capability is crucial for maintaining the system's integrity and protecting users from potentially misusing compromised or outdated credentials.
    \item[\textbf{(R4)}] Immutable Record-Keeping. The system must maintain immutable records to ensure credentials' status integrity and authenticity. Immutability is fundamental to prevent unauthorized modifications and ensure the credential status' trustworthiness. 
    \item[\textbf{(R5)}] Scalable Credential Status Management. The system must be capable of scalable management to accommodate the increasing volume of digital credentials and users.
    \item[\textbf{(R6)}] Interoperability. The system must ensure seamless interoperability within the decentralized framework across various systems and platforms.
\end{enumerate}

The methodology used in this paper involves a comparative analysis between centralized and decentralized PKI systems for managing and revoking digital credentials. This approach juxtaposes traditional mechanisms such as Certificate Revocation Lists (CRLs) and Online Certificate Status Protocol (OCSP) against blockchain-based decentralized methods. It incorporates advanced cryptographic techniques like Zero-Knowledge Proofs (ZKPs), Homomorphic Encryption (HE), and Multi-Party Computation (MPC) to examine their impact on the efficacy and reliability of decentralized credential status management. This comparative framework is designed to reveal gaps in traditional systems, evaluate decentralized credential status management systems, and forecast future developments in digital identity verification.

This paper systematically explores the evolution and implications of credential status management. Section 2 delves into the development of Public Key Infrastructure (PKI), tracing its journey from traditional centralized frameworks to decentralized models. Section 3 contextualizes traditional PKI mechanisms within emerging decentralized frameworks, assessing the adaptation and functionality of components such as CRLs and OCSP. Section 4 is dedicated to examining Decentralized Credential Status Management Systems, highlighting their role in enhancing digital security and autonomy, and exploring blockchain technology and cryptographic methods in revolutionizing credential verification and identity management.

Evaluation description!!!
This paper contributes to Decentralized Credential Status Management, particularly in the context of verifiable credentials and blockchain technology.

\begin{itemize}
    \item Comparative analysis: We comprehensively compare centralized and decentralized systems for credential management, highlighting the limitations of traditional systems and the potential of decentralized approaches.
    \item Technological Integration: Our study integrates advanced cryptographic techniques such as Zero-Knowledge Proofs (ZKPs), Homomorphic Encryption (HE), and Multi-Party Computation (MPC) in the context of DCSM, showcasing their impact on improving privacy and security.
    \item Practical Framework: We propose a practical framework for DCSM that addresses key challenges such as privacy, user-centric control, real-time revocation mechanisms, and immutable record keeping.
    \item Future-Oriented: Our research predicts the development of digital identity verification and credential management, setting a path for continued innovation in this rapidly evolving field.
\end{itemize}

% Describe the GAP

% TODO Include key management
% PGP and Web of Trust
% Accumulators The use of cryptographic accumulators as a decentralized alternative to digital signatures was first described in 1994 by Benaloh and de Mare [4].
% https://eprint.iacr.org/2014/803.pdf
% certifi cate transparency by Google

% What is a credential?
% A credential is a trust provider's statement about a thing or a person that is relied upon by other parties [79]
% Eric R. Verheul. "Self-Blindable Credential Certificates from the Weil Pairing". In: Advances in Cryptology - ASIACRYPT 2001, 7th International Conference on the Theory and Application of Cryptology and Information Security, Gold Coast, Australia, December 9-13, 2001, Proceedings. Ed. by Colin Boyd. Vol. 2248. Lecture Notes in Computer Science. Springer, 2001, pp. 533–551. isbn: 3-540-42987-5 (cit. on pp. 7, 9, 44, 83).

% Unlinkable unlinkable credentials. Among them are complete systems like U-Prove [18] and Idemix [21]. https://fse.studenttheses.ub.rug.nl/9777/1/thesis.pdf

% Definition 4.2 (Anonymity [66]). Anonymity is the state of being not identifiable within a set of subjects, the anonymity set. Anonymity of a subject from an attackers perspective means that the attacker cannot sufficiently identify the subject within the anonymity set.  Andreas Pfitzmann and Marit Hansen. A terminology for talking about privacy by data minimization: Anonymity, Unlinkability, Undetectability, Unobservability, Pseudonymity, and Identity Management. v0.34. Aug. 2010. URL: http://dud.inf.tu-dresden.de/literatur/Anon\_Terminology\_v0 .34.pdf (cit. on pp. 56, 57).


% Accumlators:
% https://fse.studenttheses.ub.rug.nl/9777/1/thesis.pdf

\section{Evolving Digital Trust: The Role of Decentralization in Public Key Infrastructure (2.5 pages)}
%
% 15.2.2024
% 
% TOSO: Work on Table and Timeline for centralized and decentralized topics with certificates, CAs, roots, intermediates
% TODO: Citations missing
%

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/2_timeline_70-2010.pdf}
    \caption{Chronological Progression and Divergence of Centralized and Decentralized Public Key Infrastructure (PKI) from the 1970s to the 2010s. The timeline provides a comparative perspective of milestones in the history of PKI. It underscores the evolving challenges and responses that have defined the field, from initial trust establishment to integrating advanced cryptographic mechanisms in centralized and decentralized contexts.}
    \label{fig:pkitimeline}
\end{figure*}

In the digital era, the expansion of online interactions necessitates robust trust mechanisms to protect privacy and ensure data integrity~\cite{weise2001public}. Traditionally, centralized trust models, anchored by Certificate Authorities (CAs), have been instrumental in digital security. However, centralized trust models are prone to vulnerabilities such as single points of failure and scalability issues~\cite{serrano2019complete}. 

The beginning of blockchain technology indicates a paradigm shift toward decentralized systems, promising enhanced security, transparency, and user empowerment in digital identity management~\cite{nakamoto2008bitcoin}. The evolution of blockchain signifies a transformative shift from centralized to decentralized trust mechanisms, heralding a new era of digital interactions characterized by increased security and user control over digital identities~\cite{swan2015blockchain}.

This Section delves into the evolution of digital trust models, tracing its journey from centralized origins towards a decentralized future. It critically examines how decentralization addresses the limitations of centralized systems, fostering a more resilient and scalable digital infrastructure. Through this exploration, this Section discusses decentralized approaches' transformative potential in redefining the digital trust and security landscape.
% finish until here ->|
\subsection{History of Public Key Infrastructure}
Public Key Infrastructure (PKI) is a security architecture that provides the foundation to establish and maintain a trustworthy digital environment. It is not a single system, but a comprehensive framework that includes standards, protocols, software, encryption technologies, and services that enable secure communications and network transactions. PKI manages, distributes, and verifies digital certificates, which bind public keys with identities of entities such as people, organizations, or devices. These digital certificates ensure that public keys are authentic, facilitating secure data exchange, digital signatures, and encryption on the Internet.

The development of PKI has experienced a transformation since its inception, marking a fundamental shift in the landscape of digital security. PKI, which laid the foundation for modern cryptographic practices, was initiated by Diffie-Hellman~\cite{1055638} key exchange in 1976, introducing the possibility of secure key exchange over insecure channels. Following Diffie-Hellman key exchange, the introduction of the Rivest–Shamir–Adleman~\cite{10.1145/359340.359342} (RSA) algorithm in 1978 propelled the evolution of secure digital communication. The RSA algorithm established a comprehensive framework for encryption and digital signatures, facilitating secure data transmission and authentication processes essential to contemporary digital security measures.

In the early 1980s, David Chaum's contributions marked a pivotal digital security and privacy shift, particularly with his 1982 paper, "Blind signatures for untraceable payments." This work introduced the concept of digital cash, which is fundamental to cryptographic privacy in digital financial transactions. Chaum proposed using blind signature schemes to maintain transaction anonymity, allowing payments without identity disclosure to banks or third parties. Despite its transformative potential, the concept faced hurdles such as underdeveloped digital infrastructure, limited public knowledge of cryptographic principles, and resistance from traditional financial institutions concerned about regulatory implications.
Chaum's vision expanded in 1985 with the proposal of a proto-blockchain protocol in "Security without Identification: Transaction Systems to Make Big Brother Obsolete," advocating for a decentralized system to secure and anonymize digital transactions against central authority surveillance. Despite its innovative approach, the realization faced limitations and societal reluctance toward disruptive technologies. Chaum's early works highlight his seminal role in digital trust and privacy and underscore the challenges in navigating the advancement of cryptographic innovations within a context of technological constraints and societal readiness. Chaum's contributions laid crucial groundwork for the privacy-preserving technologies and decentralized systems integral to modern digital infrastructure.

The late 1980s marked a period in digital security with the introduction of the X.509~\cite{x509} standard, which was instrumental in operationalizing and standardizing cryptographic technologies. The X.509 standard established a comprehensive framework for digital certificates and identity verification systems, becoming a cornerstone of PKI. Integral to the effectiveness of the X.509 standard were cryptographic algorithms such as Rivest-Shamir-Adleman~\cite{elgamal1985public},~\cite{schnorr1990efficient},~\cite{10.1145/359340.359342} (RSA), Digital Signature Algorithm (DSA)~\cite{schneier1995applied}, and Elliptic Curve Cryptography~\cite{koblitz2000state} (ECC), which provided the mechanisms for secure digital signatures and key exchanges. 
% citations missing ->
The rise of Certificate Authorities (CAs) highlighted their critical roles in issuing, managing, and revoking digital certificates, positioning them as central figures in centralized PKI. The involvement of CAs became instrumental in safeguarding the integrity and trustworthiness of digital communication channels. During this era, the introduction of Intermediate Certificate Authorities improved the scalability and reliability of digital trust mechanisms. By distributing the certification responsibilities across a network of entities, intermediaries played a crucial role in strengthening the robustness and resilience of PKIs.
Furthermore, establishing the PKIX working group~\cite{ietfpkix} by the Internet Engineering Task Force (IETF) represented a step forward in standardizing PKI protocols. This effort reflected a growing sophistication in understanding digital trust and underscored the pressing need for a more systematic and secure management of cryptographic keys. As a result, the PKIX working group was crucial in developing comprehensive PKI systems that underpin the secure digital transactions that we rely on today.
% TODO: Adding challenges to mentioned topics and Citations
During the 1990s and 2000s, as the Internet became central to global communication, PKI experienced an expansion to ensure the security of this burgeoning digital landscape. The Secure Sockets Layer (SSL) protocol, introduced in the mid-1990s, and its successor, Transport Layer Security (TLS), became fundamental for securing Internet communications, laying the groundwork for encrypted data exchange. These protocols, which depend on PKI for authentication and encryption, underscored the importance of digital certificates in establishing secure connections. In response to the increasing demand for digital certificates, Proxy Certificate Authorities have emerged as a solution that streamlines certificate issuance and management. Acting on behalf of traditional CAs, Proxy CAs offered a mechanism for more flexible and immediate certificate services, especially in environments requiring rapid or automated certificate issuance. 
However, the increased issuance of digital certificates highlighted the need for more effective revocation mechanisms. Although useful, Certificate Revocation Lists (CRLs) faced scalability and latency challenges as they became larger and more complex. In response, developers introduced the Online Certificate Status Protocol (OCSP) in 1991 to enable real-time verification of certificate statuses. Despite the OCSP improving the timeliness of revocation checks, it also brought new challenges, including higher network latency and privacy concerns for queries about individual certificates.
% TODO: Adding also the challenges to PGP
Amidst the rapid evolution of PKI during the 1990s and the increasing reliance on centralized systems for digital security, Phil Zimmermann introduced Pretty Good Privacy (PGP)~\cite{zimmermann1995official}, offering a decentralized alternative to traditional PKI systems. PGP was developed to facilitate secure communication over the Internet for individuals and groups demanding confidentiality and authentication without centralized control. The PGP initiative emerged due to trust concerns over digital surveillance and the potential for centralized authority abuse within certificate authorities~\cite{502679}. The decentralized trust model of PGP, the Web of Trust~\cite{khare1997weaving}, contrasts with the hierarchical trust model of conventional PKI. Rather than relying on central authorities for identity validation, PGP enables users to sign and exchange keys within a trusted network, allowing peer verification and trust level assignments to determine public key authenticity. This decentralized ethos inherent in PGP's architecture provided a foundation for developing alternative trust models in digital credential management, emphasizing user control over cryptographic keys and the direct management of trust relationships. By enabling individuals to create, distribute, and revoke their encryption keys without centralized certificate authorities, PGP demonstrated a model for securing digital communications operating independently of the traditional PKI framework. The PGP methodology gave users greater autonomy in managing their digital identities, subsequently influencing the development of innovations in decentralized identity and credentialing systems. Consequently, establishing PGP's principles signifies a landmark event in advancing cryptographic practices. The principles established in PGP provide valuable information for the creation of modern systems that aim to harmonize security, privacy, and user independence within decentralized frameworks.

At the same time, foundational concepts emerged for modern blockchain technology, marking milestones in the cryptographic landscape. In 1991, Stuart Haber and W. Scott Stornetta proposed a secure method of timestamping digital documents, which would later be recognized as a precursor to blockchain technology. Enhancements such as Merkle trees in 1992 by Haber and Stornetta and Adam Back's Hashcash proof-of-work system in 1997 further advanced the efficiency and security of decentralized digital systems. These early innovations laid the groundwork for the distributed ledger technologies that underpin modern cryptocurrencies and decentralized applications, demonstrating the growing interest in alternative trust models beyond the centralized PKI framework.

The PGP initiative and the development of early blockchain concepts reflect a shared concern about digital surveillance and the potential for abuse within centralized systems. By emphasizing user control over cryptographic keys and direct management of trust relationships, both movements provided a foundation for developing alternative trust models in digital credential management. These efforts underscored the complexity of transitioning to a decentralized framework while ensuring robust security and user-friendly experiences. Furthermore, they highlighted the ongoing need for solutions that balance security, privacy, and usability in decentralized contexts, providing essential insight into the potential and pitfalls of decentralized PKI systems.
% citations missing
% TODO: Citation and more challenges regarding CRL and OCSP? Certificate usage? HTTPS? EMAIL Documents? 
From the 2000s to today, centralized PKI has seen innovations that address previous limitations and adapt to new technological landscapes. The Automatic Certificate Management Environment (ACME) automates the acquisition, renewal, and deployment of digital certificates, and eases the management burden of PKI operations~\cite{Barnes2019AutomaticCM}. Despite its advantages, ACME requires assistance with broad adoption and securing automated processes~\cite{bhargavan2017formal}. Integrating Certificate Transparency (CT) in PKI improves security by implementing public logging and verification of certificates~\cite{10.1145/2659897}. This approach addresses centralization vulnerabilities, strengthening trust, and mitigating risks such as Certificate Authority compromise and man-in-the-middle attacks. The evolution to CT Version 2.0~\cite{laurie2021certificate} refines the protocol to address the dynamic challenges in digital certificate management. By introducing enhancements such as algorithm agility and a streamlined approach for logging certificates, CT 2.0 aims to secure a PKI against vulnerabilities further. Despite the security enhancements introduced by CT and its evolution to CT Version 2.0, challenges persist. While addressing certain vulnerabilities, reliance on a centralized logging system introduces potential operational fragilities and privacy concerns. Specifically, the public exposure of logged certificates can inadvertently reveal domain names, presenting privacy issues and potentially aiding malicious actors in identifying targets for cyber attacks~\cite{10.1145/3278532.3278562}. 

The development of OCSP led to the advent of OCSP Stapling~\cite{wazan2020validation}, which improved the verification process of the certificate status in real time. By incorporating the OCSP response directly into the TLS handshake, OCSP Stapling successfully mitigated the privacy and latency issues associated with the conventional OCSP, thereby improving the efficiency of the certificate verification process. The advancement of OCSP Stapling allowed clients to authenticate certificates without needing to verify their status through CAs directly. Although OCSP Stapling improved efficiency and privacy, it also exposed certain limitations, notably certificate chain validation and "soft failure" scenarios, where clients may accept certificates without accessing revocation information~\cite{10.1145/3419394.3423664}. To address these shortcomings of OCSP Stapling, the OCSP Must-Staple~\cite{chung2018web} extension was introduced, mandating a valid OCSP response for the TLS handshake and implementing stricter security protocols. However, the adoption of OCSP Must-Staple has progressed gradually, highlighting the challenges in balancing improved security and efficiency with widespread implementation in the digital certificate ecosystem. The difference between OCSP Stapling and OCSP Must-Staple rests in their approach to enforcement; OCSP Stapling provides a mechanism for disclosing revocation data, whereas OCSP Must-Staple enforces strict compliance with this protocol, thereby strengthening the security framework through exhaustive checks on revocation status.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/2_timeline_20-24.pdf}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}
%Citations? 
Parallel to these developments in centralized PKI, the mid-2000s to 2009 marked advancements in the evolution of decentralized technologies. In 2004, Hal Finney introduced Reusable Proof of Work (RPOW). In this system, proof-of-work tokens could be exchanged between individuals, demonstrating a concept that would later become integral to Bitcoin's proof-of-work mechanism. This period also saw the rise of decentralized platforms like BitTorrent, which became mainstream by 2005-2007, illustrating the practical applications of decentralized networks in peer-to-peer file sharing. The pivotal moment came in 2008 when Satoshi Nakamoto published "Bitcoin: A Peer-to-Peer Electronic Cash System," introducing the first blockchain implementation and proposing a solution to the double-spending problem without needing a trusted authority. The launch of Bitcoin in 2009, with the mining of the genesis block in January, signaled the practical inception of decentralized cryptocurrencies. These developments underscored the potential of blockchain technology to create secure, decentralized systems for digital transactions and identity management. However, the evolution of digital trust and identity management has also been marked by the advent of decentralized technologies, which have introduced new paradigms in how digital identities and credentials are created, verified, and managed.

The introduction of Smart Contracts and Decentralized Autonomous Organizations (DAOs) has revolutionized the automation of processes and the governance of decentralized systems. These technologies have enabled more efficient and trustless interactions within blockchain networks, impacting decentralized PKI systems by facilitating automated issuance, revocation, and management of digital certificates without centralized control. This shift towards automation and decentralized governance models reflects a broader movement towards self-sovereignty and user-centric digital identity solutions. Interoperability protocols such as Polkadot and Cosmos and Layer 2 scaling solutions have addressed key challenges of scalability and cross-chain communication, ensuring that decentralized applications can operate efficiently and seamlessly across different blockchain networks. These advancements are essential for the widespread adoption and practical implementation of decentralized systems, including decentralized PKI and identity management platforms.
% citations missing 2010 -> 2020 -> 2030 
Following advancements in digital identity technologies, the emergence of Self-Sovereign Identity (SSI) has catalyzed a paradigm shift in how individuals manage and control their digital identities. Rooted in the principles of decentralization, SSI offers individuals unparalleled control over their personal information, free from the oversight of centralized authorities. This transformative approach to digital identity management is founded on developing Decentralized Identifiers (DIDs) and Verifiable Credentials (VCs), which together form the cornerstone of SSI systems. DIDs and VCs enable a more secure, private, and interoperable framework for digital identities, perfectly aligning with the ethos of SSI by enhancing user autonomy in the digital realm and promoting privacy-preserving interactions.

Cryptographic innovations such as zero-knowledge proofs (ZKPs) in the 1980s have played a central role in this shift, offering a method to prove a claim's authenticity without compromising the underlying data's privacy. These technologies promise enhanced privacy and security and mark a new era of user control and autonomy over digital identities. However, the transition toward SSI presents challenges, including the need for widespread adoption, overcoming interoperability hurdles, and the development of user-friendly interfaces. There is a pressing need for seamless integration of SSI solutions into existing digital ecosystems to fully realize their potential.
The journey from concept to implementation of SSI exemplifies the broader movement towards decentralized systems, highlighting the evolving nature of digital trust and the ongoing search for solutions prioritizing user control and privacy. By incorporating foundational technologies such as DIDs, VCs, and ZKPs, this movement supports a secure and private foundation for establishing decentralized digital identities, signaling a leap forward in the quest for a more secure, user-centric, and self-sovereign digital future.

Integration of advanced cryptographic technologies into SSI, namely Zero-Knowledge Proofs (ZKPs), Multiparty Computation (MPC), Fully Homomorphic Encryption (FHE), and quantum-resistant cryptography, has enhanced the privacy and security landscape of decentralized systems. These technologies offer sophisticated methods for protecting data and ensuring the integrity of digital transactions, which are particularly crucial in decentralized identity management. ZKPs enable the verification of information without revealing the actual data, thus preserving privacy and ensuring authenticity. This is particularly relevant for SSI, where individuals can prove their identity or permissions without exposing sensitive personal information. MPC allows multiple parties to compute outcomes based on their combined data without actually sharing the data among themselves, facilitating collaborative yet confidential verification processes. FHE takes this further by allowing operations on encrypted data, ensuring that user data remains secure even during processing. Lastly, as the potential of quantum computing looms, quantum-resistant cryptography prepares the digital security infrastructure to withstand future threats, safeguarding digital identities against unprecedented computational capabilities.

These cryptographic advances form a critical component of the SSI framework, which addresses some of the most pressing challenges in privacy, security, and interoperability. They enhance the trustworthiness of decentralized digital identities and ensure that these systems are resilient against evolving cyber threats. Integrating these technologies into SSI solutions marks a pivotal development in the journey toward a secure, privacy-preserving, and user-centric digital world. The ongoing refinement and adoption of these cryptographic techniques will be instrumental in overcoming the existing barriers to SSI adoption. This will facilitate a seamless transition to a decentralized identity ecosystem that prioritizes user control, privacy, and security.

Parallel to the development of SSI, the 2010s also witnessed the introduction of blockchain-based Certificate Transparency (CT) logs. These logs leveraged blockchain technology's inherent transparency and immutability to enhance the security and verifiability of certificate issuance records. Blockchain-based CT logs aim to address vulnerabilities associated with centralized CAs, including misissuance and fraud, by creating a publicly accessible and tamper-evident ledger of digital certificates. Despite its potential, the integration of blockchain technology into CT systems faced challenges related to scalability, as the size and frequency of transactions lead to congestion and increased latency on the blockchain. Additionally, the balance between transparency and privacy emerged as a critical concern, necessitating innovative solutions to protect sensitive information while maintaining an open and verifiable record of certificate issuances.
% TODO add Zero Knowlege Proof, MPC, FHE
Exploring Decentralized Public Key Infrastructure (DPKI) protocols marked another advance in this period. DPKI sought to use blockchains and other distributed systems to democratize the issuance and revocation of digital certificates, thus eliminating central points of failure and improving security. The adoption of DPKI posed challenges in achieving consensus on the validity of certificates and the revocation process in a decentralized environment. Establishing trust without a centralized authority required robust mechanisms for consensus and verification, which in turn necessitated computational resources and innovative algorithmic solutions. Moreover, the transition from traditional PKI to DPKI systems raised questions about compatibility and coexistence, as the digital ecosystem had to accommodate both centralized and decentralized trust models during this transitional phase.

\input{tables/2_summary}


Building on the history of central and decentralized PKI systems, it becomes evident that while centralized PKI architectures have been instrumental in establishing digital trust and security, they possess vulnerabilities that can undermine the very fabric of secure online communications. The exposition of central PKI systems' limitations, ranging from single points of failure and scalability issues to challenges in certificate revocation and management, lays the groundwork for the exploration of decentralized approaches. As the digital landscape evolves, so does the need for a more robust, scalable, and user-centric model of trust. This realization brings us to this Systematization of Knowledge research: The exploration of Decentralized Credential Status Management (DCSM). The transition towards DCSM not only aims to address the shortcomings of traditional PKI but also seeks to leverage the advancements in blockchain technology and cryptographic innovations to develop a new path for digital identity verification and trust. This evolution from centralized to decentralized systems underscores a broader shift towards enhancing web security, ensuring user privacy, and facilitating real-time verification of digital certificates, marking a more secure and self-sovereign digital future.

% TODO: READS UNTIL HERE !!! CITATIONS

\input{tables/2_comparison}
% text finish until here, citations missing ->|
% What has centralized and decentralized PKI todo with decentralized credential status management? 

\subsection{Key Management and Certificates}
Private and public keys, along with digital certificates, are the building blocks of centralized PKI. PKI enables secure and encrypted communication between authenticated parties, ensuring the protection of sensitive data against unauthorized access~\cite{Housley2002InternetXP}. CAs play a crucial role in PKI, as they are the trusted entities responsible for issuing and verifying digital certificates~\cite{6547130}. These certificates serve as verifiable links between public keys and their rightful owners, whether individuals or machines, enabling these entities to assert their digital identities and establish credibility within the digital realm. The certificate issuance process starts with Domain Validation (DV)~\cite{bhargavan2017formal}, where a CA verifies the applicant's control over a domain, offering a basic security level. The next level, Organization Validation (OV)~\cite{vratonjic2013inconvenient}, involves a more detailed check, confirming an organization's legal existence when applying for a certificate. The most comprehensive level, Extended Validation (EV)~\cite{jackson2007evaluation},~\cite{thompson2019web}, includes an in-depth review of the organization's identity and legal status. 

Each step in the hierarchical validation process aims to ensure that digital certificates are allocated to verified entities. However, PKI validation processes transitions into security vulnerabilities, especially within centralized systems.

%Security Considerations and Challenges: Address the security vulnerabilities inherent in centralized PKI, such as the risk of CA compromise, man-in-the-middle attacks, and the implications of single points of failure. Discuss the implications of these vulnerabilities and the importance of robust security practices.

Schwittmann et al.~\cite{8806745} reveal vulnerabilities in the CA domain validation processes, showing how attackers can obtain certificates for domains they do not own. The research from Schwittmann et al. highlights the reliance on insecure protocols like Domain Name System (DNS) and HTTP, without implementing secure alternatives such as DNS Securtiy Extenstion (DNSSEC)~\cite{chung2017understanding} and Transport Layer Security (TLS)~\cite{turner2014transport}. All tested CAs exhibited vulnerabilities in various degrees, indicating a fundamental weakness in web security. The paper suggests improvements for domain owners and CAs to enhance security and mitigate these vulnerabilities. Brandt et al.~\cite{10.1145/3243734.3243790} uncover vulnerabilities in the domain validation process, where attackers can falsely validate domain ownership without direct access to communication paths. Vulnerabilities in domain validation allow attackers to obtain certificates for domains they do not control, exploiting weaknesses in DNS resolution processes. Brandt et al. emphasize the risk of relying on insecure validation methods and propose more secure validation strategies to mitigate vulnerabilities. 

When attackers exploit vulnerabilities in the certificate issuance process to acquire unauthorized certificates, immediate revocation is crucial. Authorities must invalidate "compromised" certificates before their scheduled expiration, preventing their use in secure communications. Revocation is crucial in preserving the integrity of secure communication channels. The management of such revocation processes, through mechanisms like CRLs and the OCSP, allows users to verify the revocation status of certificates. The forthcoming section contextualizes centralized and decentralized methods for managing certificate statuses, highlighting the distinctions between revocation, suspension, and the reactivation of credentials.

We encounter notable security considerations as we navigate the intricacies of centralized PKI, including its rigorous processes for certificate issuance, management, and revocation. These systems, centralized around Certificate Authorities (CAs), introduce vulnerabilities such as potential single points of failure. A compromise within a CA affects the integrity of numerous digital certificates and the security fabric of countless encrypted communications and transactions. Moreover, the operational challenges of certificate revocation and the centralized trust model necessitate reevaluating the mechanisms underpinning digital trust.

\subsection{Decentralization of Trust}

In decentralized systems, trust is distributed throughout the network, mitigating the risk associated with dependence on a singular centralized authority. Such an architectural shift enhances the system's resilience, transparency, and adaptability, fostering a robust trust ecosystem. Decentralized systems can encompass diverse entities, including virtual organizations that converge on consensus mechanisms, consortia responsible for issuing verifiable credentials, and educational networks tasked with distributing student identifiers. Participants within these decentralized networks may comprise organizations, educational institutions, or non-profit organizations. Transitioning to a decentralized framework reduces the vulnerability associated with a single point of failure, thereby augmenting the system's security and ensuring greater transparency. In contrast, centralized Public Key Infrastructure (PKI) systems centralize trust within specific entities, increasing susceptibility to targeted attacks and presenting a singular point of compromise. Decentralized systems, by distributing trust, eliminate this central point of failure and enhance security through redundancy and consensus-driven validation mechanisms. Furthermore, decentralized frameworks facilitate interoperability and self-sovereignty, enabling entities to directly control and verify credentials without intermediaries.

However, the dynamic and evolving digital landscape necessitates a paradigm shift towards more resilient, flexible, and decentralized trust models. This section comprehensively explores PKI evolution, critically analyzing the design principles, operational modalities, and inherent challenges of centralized and decentralized PKI architectures. Our journey through the PKI domain aims to illuminate the transformative potential of decentralization in redefining digital trust and security frameworks.

The discourse examines key management practices following the discussion of Self-sovereign Identity (SSI). It focuses on established centralized key management systems, elucidating their architecture and security protocols. The Key management analysis serves as a precursor to exploring decentralized key management strategies, thereby establishing a context for the subsequent analysis of certificate and credential revocation mechanisms within these frameworks.

\subsection{Key Management Across Models}
%Traditional vs. Decentralized Key Management: Compare key management in centralized and decentralized systems. Challenges and Innovations in Key Management: Explore how decentralized PKI addresses key management challenges.

Key management in PKI systems is crucial to the security and integrity of cryptographic operations. This subsection delves into the principles and practices that govern key PKI management. We focus on the mechanisms employed to generate, distribute, store, and revoke cryptographic keys.

\textit{Key Generation:} The cornerstone of PKI key management is the generation of cryptographic keys. This process must adhere to stringent security protocols to ensure the robustness of the keys. Dealing keys involves creating pairs of public and private keys using cryptographic algorithms. The strength and security of these keys are pivotal, as they underpin the entire PKI system.

After being generated, the distribution of keys, especially public keys, becomes a focus.CAs issue digital certificates in PKI to distribute public keys. Certificates bind a public key to the identity of the corresponding entity, ensuring the legitimacy of the claimed representation. This process of binding and associating public keys with specific identities maintains trust within the PKI framework by verifying the authenticity of the identity-key pairing. Pairing identity keys is essential to ensure the security infrastructure's effectiveness. Digital certificates serve a critical function by associating a public key with a specific entity's identity. This association confirms that the public key corresponds to the entity it purports to represent. Such a binding mechanism is essential in preserving and fostering trust within the PKI framework, ensuring the integrity of the identity-key relationship and thus maintaining the security infrastructure's overall efficacy.

Digital certificates bind a public key with an identity, ensuring that it belongs to the entity it claims to represent. In addition to key generation and distribution, it is essential to store and access cryptographic keys securely. This aspect is critical to maintaining the confidentiality and integrity of keys throughout their lifecycle. The following subsection explores strategies and practices for secure key storage and accessibility within PKI systems.

\textit{Key Storage and Accessibility:} The security and accessibility of cryptographic keys, particularly private keys, are crucial in PKI systems. Key storage techniques include hardware security modules (HSM) and trusted execution environments (TEE). In PKI, secure storage and accessibility of cryptographic keys, especially private ones, are paramount. Hardware Security Modules (HSMs) provide a secure hardware environment for key storage, protecting against physical and logical attacks. They handle cryptographic operations within the module, minimizing exposure, and enhancing security. Trusted Execution Environments (TEEs) provide another layer of security, offering isolated execution spaces where sensitive operations and data can be processed and stored, shielded from the operating system. This isolation helps prevent unauthorized access and tampering, making TEEs a valuable asset in key management strategies. Both HSMs and TEEs represent advanced technologies in key storage and accessibility, ensuring that cryptographic keys remain secure, yet accessible for authorized use within PKI frameworks. The discussion progresses to another key management aspect: Key Revocation. The following subsection will explore the mechanisms and importance of revoking keys within PKI.

\textit{Key Revocation in PKI:}
Key revocation protects the security and trustworthiness of a system. Revocation of keys involves invalidating digital certificates that are compromised, declared invalid, or have limited associated credentials. The importance of key revocation is ensuring that the circulating certificates are secure and valid.
Digital certificates authenticate identities and establish trust in online environments. The ability to revoke digital certificates is a requirement and a crucial aspect of maintaining secure digital communications and transactions. Therefore, the key revocation process directly impacts the PKI trust model, affecting how entities within the system interact and trust each other.

The forthcoming section in this SoK paper will delve into methodologies and mechanisms used for key revocation in PKI systems, focusing mainly on certificate revocation lists (CRL) and the online certificate status protocol (OCSP). This exploration will examine the functions of these mechanisms in the broader spectrum of certificate management and PKI security. In the context of this paper's primary research direction – the shift from centralized to decentralized credential status management systems – key revocation mechanisms are pivotal elements. This analysis will illustrate how traditional revocation methods are adapted, or potentially reenvisioned, in decentralized systems, such as those based on blockchain technology.

\subsection{Comparative Analysis: Centralized vs. Decentralized PKI}
Transition Challenges and Opportunities

% Conclusion
% Summarize the insights on the evolution from centralized to decentralized PKI. Emphasize the significance of this transition in the broader context of digital security and identity management.
% List of abbreviations

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Public Key Infrastructure (PKI) is crucial in digital security, entity authentication and communication integrity over the Internet~\cite{maurer1996modelling}. This section explores the evolution of PKI from its traditional, centralized framework, dominated by Certificate Authorities (CAs), to evolving decentralized systems. It underscores the foundational significance of the X.509 standard and investigates the transformative impact of integrating blockchain and other decentralized technologies. By critically examining the inherent challenges in traditional PKI systems, such as scalability constraints and vulnerability to single points of failure, the section prepares the ground for assessing the efficacy of decentralized approaches in enhancing digital security, transparency, and user centricity. The following analysis aims to illuminate the complexities and potential trajectories in the evolution of PKI.

\subsection{The Evolution and Current Landscape of PKI}
The Public Key Infrastructure (PKI) stands as a cornerstone in the domain of digital security, indispensable for the validation and management of digital certificates. X.509 certificates, in particular, play a pivotal role in authenticating entities across the Internet. The PKI framework, which includes cryptographic keys and mechanisms, enables secure encrypted exchanges between entities on unsecured networks. It is instrumental in guaranteeing the confidentiality and integrity of digital interactions, substantiating the authenticity of certificate holders. Central to PKI's function is effectively managing and safeguarding cryptographic keys, underlining its critical role in sustaining digital security.

\textbf{Centralized PKI Systems and the Role of Certificate Authorities. } In traditional PKI systems, Certificate Authorities (CAs) verify the identities of entities (holders) before issuing digital certificates. Each X.509 certificate encapsulates crucial information: the holder's public key, name, validity period, and the CA's digital signature. This verification process, underpinned by the CA's public key, is vital for accurate representation and validation of holders' identities, reinforcing the integrity of digital interactions.

\textbf{Significance of the X.509 Standard Beyond Domain Authentication. }
The X.509 standard forms the backbone of transport layer security (TLS) and HTTPS, expanding its utility beyond the web application's authentication. Its application in protocols like Secure Multipurpose Internet Mail Extensions (S/MIME) for encrypted email communications and systems such as LDAP and XMPP demonstrates its versatility and indispensability in the broader context of digital security. X.509's adaptability across various digital security protocols highlights its comprehensive role in securing digital documents and managing digital identities.

\subsection{Challenges and Limitations of Traditional PKI Systems}
Traditional PKI systems face challenges mainly due to their reliance on centralized certificate authorities (CA). A centralized structure introduces risks of single points of failure and presents scalability challenges, particularly evident in the certificate revocation process. Managing a certificate's lifecycle, encompassing issuance to revocation and verification, necessitates a critical reevaluation and adaptation of conventional methods, aligning them with the evolving requirements of digital security paradigms.

\textit{Scalability and Certificate Revocation Processes.} A primary challenge in centralized PKI systems is the scalability of certificate revocation processes. The increasing issuance of digital certificates in the evolving digital landscape strains existing revocation mechanisms like CRLs and OCSP. This scalability issue manifests itself in delays in revocation updates and imposes an overhead on network resources, compromising operational efficiency.

\textbf{Critical Reevaluation of Conventional PKI Methods. } In light of the challenges mentioned, there is a need for a critical re-evaluation and adaptation of traditional PKI methodologies. Such an adaptation should focus on enhancing the scalability and reliability of these systems. It should also aim to improve PKI's overall security framework to keep pace with the dynamic and evolving nature of digital security threats and demands.

\textbf{Potential of Decentralized Systems as Alternatives. } Emerging decentralized technologies, notably blockchain, present a paradigm shift from the traditional centralized trust model. Decentralized systems propose a framework for managing digital certificates, offering enhanced security, transparency, and scalability. These systems use distributed ledger technologies and consensus algorithms to democratize control and distribute trust across a network, mitigating centralization risks.

As we conclude our examination of the evolution and current challenges within traditional PKI systems, we are at the threshold of a new frontier in digital security. The following section, "Contextualization of Traditional PKI Mechanisms within Decentralized Frameworks," will explore how these time-tested mechanisms can be reimagined within decentralized technologies. This section aims to bridge the conceptual gap between the established centralized PKI processes and the innovative decentralized models, mainly focusing on how blockchain and similar technologies can enhance or transform traditional practices like CRLs and OCSP. We will critically analyze the potential synergies, as well as the challenges, that arise when melding these two seemingly disparate worlds. The forthcoming discourse promises to offer insightful perspectives on the future trajectory of PKI, where the fusion of the old and the new could redefine the paradigms of trust and security in the digital realm.

The following section, Decentralized Credential Status Management, focuses on how traditional PKI mechanisms are adapted and reimagined in decentralized frameworks, particularly in managing and verifying digital credentials in a decentralized environment.

% Subsequently, the intersection of PKI and Content Delivery Networks (CDNs) is explored. This examination is vital as CDNs, integral to the global internet infrastructure, rely on PKI to distribute content securely. 

% Section 2 intro deleted
%In the digital era, the expansion of online interactions necessitates robust trust mechanisms to protect privacy and ensure data integrity~\cite{weise2001public}. Centralized trust models, anchored by Certificate Authorities (CA), have been instrumental in digital security. However, centralized trust models are prone to vulnerabilities such as single points of failure and scalability issues~\cite{serrano2019complete}. 

DCSM Section Backup

\section{Opportunities with Decentralized PKI}
The introduction of Smart Contracts and Decentralized Autonomous Organizations (DAOs) has revolutionized the automation of processes and the governance of decentralized PKI systems. These technologies have enabled efficient and trustless interactions within blockchain networks, impacting decentralized PKI systems by facilitating automated management of digital certificates without centralized control. This shift towards automation and decentralized governance models reflects a broader movement towards self-sovereignty and user-centric digital identity solutions. Interoperability protocols such as Polkadot and Cosmos and Layer 2 scaling solutions have addressed key challenges of scalability and cross-chain communication, ensuring that decentralized applications can operate efficiently and seamlessly across different blockchain networks. These advancements are essential for the widespread adoption and practical implementation of decentralized systems, including decentralized PKI and identity management platforms.



\input{tables/2_summary}


Building on the history of central and decentralized PKI systems, it becomes evident that while centralized PKI architectures have been instrumental in establishing digital trust and security, they possess vulnerabilities that can undermine the very fabric of secure online communications. The exposition of central PKI systems' limitations, ranging from single points of failure and scalability issues to challenges in certificate revocation and management, lays the groundwork for the exploration of decentralized approaches. As the digital landscape evolves, so does the need for a more robust, scalable, and user-centric model of trust. This realization brings us to this Systematization of Knowledge research: The exploration of Decentralized Credential Status Management (DCSM). The transition towards DCSM not only aims to address the shortcomings of traditional PKI but also seeks to leverage the advancements in blockchain technology and cryptographic innovations to develop a new path for digital identity verification and trust. This evolution from centralized to decentralized systems underscores a broader shift towards enhancing web security, ensuring user privacy, and facilitating real-time verification of digital certificates, marking a more secure and self-sovereign digital future.

% TODO: READS UNTIL HERE !!! CITATIONS

\input{tables/2_comparison}
% text finish until here, citations missing ->|
% What has centralized and decentralized PKI todo with decentralized credential status management? 



\subsection{Key Management and Certificates}
Private and public keys, along with digital certificates, are the building blocks of centralized PKI. PKI enables secure and encrypted communication between authenticated parties, ensuring the protection of sensitive data against unauthorized access~\cite{Housley2002InternetXP}. CAs play a crucial role in PKI, as they are the trusted entities responsible for issuing and verifying digital certificates~\cite{6547130}. These certificates serve as verifiable links between public keys and their rightful owners, whether individuals or machines, enabling these entities to assert their digital identities and establish credibility within the digital realm. The certificate issuance process starts with Domain Validation (DV)~\cite{bhargavan2017formal}, where a CA verifies the applicant's control over a domain, offering a basic security level. The next level, Organization Validation (OV)~\cite{vratonjic2013inconvenient}, involves a more detailed check, confirming an organization's legal existence when applying for a certificate. The most comprehensive level, Extended Validation (EV)~\cite{jackson2007evaluation},~\cite{thompson2019web}, includes an in-depth review of the organization's identity and legal status. 

Each step in the hierarchical validation process aims to ensure that digital certificates are allocated to verified entities. However, PKI validation processes transitions into security vulnerabilities, especially within centralized systems.

%Security Considerations and Challenges: Address the security vulnerabilities inherent in centralized PKI, such as the risk of CA compromise, man-in-the-middle attacks, and the implications of single points of failure. Discuss the implications of these vulnerabilities and the importance of robust security practices.

Schwittmann et al.~\cite{8806745} reveal vulnerabilities in the CA domain validation processes, showing how attackers can obtain certificates for domains they do not own. The research from Schwittmann et al. highlights the reliance on insecure protocols like Domain Name System (DNS) and HTTP, without implementing secure alternatives such as DNS Securtiy Extenstion (DNSSEC)~\cite{chung2017understanding} and Transport Layer Security (TLS)~\cite{turner2014transport}. All tested CAs exhibited vulnerabilities in various degrees, indicating a fundamental weakness in web security. The paper suggests improvements for domain owners and CAs to enhance security and mitigate these vulnerabilities. Brandt et al.~\cite{10.1145/3243734.3243790} uncover vulnerabilities in the domain validation process, where attackers can falsely validate domain ownership without direct access to communication paths. Vulnerabilities in domain validation allow attackers to obtain certificates for domains they do not control, exploiting weaknesses in DNS resolution processes. Brandt et al. emphasize the risk of relying on insecure validation methods and propose more secure validation strategies to mitigate vulnerabilities. 

When attackers exploit vulnerabilities in the certificate issuance process to acquire unauthorized certificates, immediate revocation is crucial. Authorities must invalidate "compromised" certificates before their scheduled expiration, preventing their use in secure communications. Revocation is crucial in preserving the integrity of secure communication channels. The management of such revocation processes, through mechanisms like CRLs and the OCSP, allows users to verify the revocation status of certificates. The forthcoming section contextualizes centralized and decentralized methods for managing certificate statuses, highlighting the distinctions between revocation, suspension, and the reactivation of credentials.

We encounter notable security considerations as we navigate the intricacies of centralized PKI, including its rigorous processes for certificate issuance, management, and revocation. These systems, centralized around Certificate Authorities (CAs), introduce vulnerabilities such as potential single points of failure. A compromise within a CA affects the integrity of numerous digital certificates and the security fabric of countless encrypted communications and transactions. Moreover, the operational challenges of certificate revocation and the centralized trust model necessitate reevaluating the mechanisms underpinning digital trust.

In decentralized systems, trust is distributed throughout the network, mitigating the risk associated with dependence on a singular centralized authority. Such an architectural shift enhances the system's resilience, transparency, and adaptability, fostering a robust trust ecosystem. Decentralized systems can encompass diverse entities, including virtual organizations that converge on consensus mechanisms, consortia responsible for issuing verifiable credentials, and educational networks tasked with distributing student identifiers. Participants within these decentralized networks may comprise organizations, educational institutions, or non-profit organizations. Transitioning to a decentralized framework reduces the vulnerability associated with a single point of failure, thereby augmenting the system's security and ensuring greater transparency. In contrast, centralized Public Key Infrastructure (PKI) systems centralize trust within specific entities, increasing susceptibility to targeted attacks and presenting a singular point of compromise. Decentralized systems, by distributing trust, eliminate this central point of failure and enhance security through redundancy and consensus-driven validation mechanisms. Furthermore, decentralized frameworks facilitate interoperability and self-sovereignty, enabling entities to directly control and verify credentials without intermediaries.

However, the dynamic and evolving digital landscape necessitates a paradigm shift towards more resilient, flexible, and decentralized trust models. This section comprehensively explores PKI evolution, critically analyzing the design principles, operational modalities, and inherent challenges of centralized and decentralized PKI architectures. Our journey through the PKI domain aims to illuminate the transformative potential of decentralization in redefining digital trust and security frameworks.

The discourse examines key management practices following the discussion of Self-sovereign Identity (SSI). It focuses on established centralized key management systems, elucidating their architecture and security protocols. The Key management analysis serves as a precursor to exploring decentralized key management strategies, thereby establishing a context for the subsequent analysis of certificate and credential revocation mechanisms within these frameworks.

The evolution from traditional certificate management towards DCSM aims to provide a scalable framework for credential management, prioritizing user-centric governance in decentralized, and digital transactions. We have identified the following requirements for DCSM as essential to adapt to evolving decentralized environments. These requirements are imperative to successfully transition to a decentralized framework, ensuring that credential management is scalable, reliable, and aligned with the increasing focus on user-centric control and privacy within decentralized interactions.

\begin{enumerate}
    \item[\textbf{(R1)}] Privacy and Untraceability. The system must ensure that unauthorized entities cannot trace user identity and activities. It should employ anonymization and privacy-enhancing technologies to preserve user confidentiality.
    \item[\textbf{(R2)}] User-Centric Control. The system must prioritize user control, allowing individuals to autonomously manage their digital identities autonomously, thus increasing user autonomy and oversight. 
    \item[\textbf{(R3)}] Real-Time Revocation Mechanisms. The system must enable efficient revocation processes, allowing immediate responses to security breaches or when credentials become invalid. This capability is crucial for maintaining the system's integrity and protecting users from potentially misusing compromised or outdated credentials.
    \item[\textbf{(R4)}] Immutable Record-Keeping. The system must maintain immutable records to ensure credentials' status integrity and authenticity. Immutability is fundamental to prevent unauthorized modifications and ensure the credential status' trustworthiness. 
    \item[\textbf{(R5)}] Scalable Credential Status Management. The system must be capable of scalable management to accommodate the increasing volume of digital credentials and users.
    \item[\textbf{(R6)}] Interoperability. The system must ensure seamless interoperability within the decentralized framework across various systems and platforms.
\end{enumerate}
% Concept and Implementation: Explain the concept of Decentralized Credential Status Management (DCSM), focusing on blockchain's role. Advantages Over Traditional Systems: Highlight how DCSM addresses the identified challenges, emphasizing privacy, scalability, and real-time verification. Requirements for DCSM: Detail the identified requirements essential for the successful transition to a decentralized framework.
\section{dcsm}
CA ist vorher eingeführt als Abkürzung für Certificate Authority - geläufiger Begriff für PKI nerds und Begriff für „Root“ Zertifikatsausteller. Aufgabe: schau mal nach, wer CA der TU Berlin website ist?
Wichtig: Root CAs sign x.509 certificates to holder or sub-CAs. Sub-CAs issuer signed certificates to domain owner. A certificate binds a verifiable a public key to domain owner or machines. Sub-CAs are also holder. They got permission for x.509 certificate signing from the root CA. Certificates can be managed by multiple issuer. A Certificate can have a trust chain from leaf owner through sub-CAs to root CA(s).
Challenge: Establish a decentralized, robust trust system. The trust system consists of a decentral network consisting of a synchronized ledger. Issuer distribute the role of root authority among these nodes and trust with agreed consensus algorithms.
Solution: established shared secretes among issuer. Signing digital documents requires at least the majority of all issuer. Our research includes multi-party computation for distributing trust among node operates and issuer.
Solution: Enhancing a shared secret multi-party framework for credential status management with fully homomorphic encryption. Fully Homomorphic Encryption (FHE) enables the execution of arbitrary computations on encrypted data without requiring access to the decryption key. This capability allows for the performance of addition and multiplication operations on ciphertexts and supports the evaluation of any computable function. Consequently, FHE facilitates secure data processing in untrusted environments, preserving the confidentiality of the underlying data while enabling complex data analyses and computation

\begin{itemize}
    \item Detailed analysis of recent advancements in decentralized credential management systems.
    \item Examination of technologies like blockchain, ZKPs, HE, and MPC in the context of revocation.
    \item Critical comparison of these technologies, focusing on their application in credential revocation.
\end{itemize}

% Contextualisation backup
\section{Contextualization of traditional PKI mechanisms within decentralized frameworks}
% Gutes SoK: paper: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8865045

This section conducts an in-depth analysis and contextualization of traditional PKI mechanisms within decentralized frameworks. It extends its focus beyond the conventional realms of Certificate Revocation Lists (CRLs) and Online Certificate Status Protocol (OCSP) to encompass a broader spectrum of mechanisms. This exploration illustrates the potential advantages and challenges of transitioning centralized mechanisms to a decentralized context.

Subsequently, the focus shifts to analyzing and evaluating decentralized credential status systems. This section strategically contextualizes traditional revocation mechanisms, comprehensively understanding their application and evolution in decentralized environments. This structured approach ensures a nuanced exploration of the theoretical and practical aspects of the significant shift in the digital security infrastructure from centralized to decentralized paradigms.

\subsection{Certificate Revocation Lists}
% TODO: QA
Certificate Revocation Lists (CRLs) serve as a foundational mechanism in Public Key Infrastructure (PKI) for the revocation of digital certificates. Certificate Authorities (CAs) actively manage and issue CRLs primarily hosted on their servers. In these lists, CAs include detailed information such as the serial numbers and revocation dates of invalidated certificates. The onus of maintaining accurate and up-to-date CRLs lies with the CAs, ensuring the reliability of revocation data.
In a typical PKI system, entities refer to the CRLs to verify a certificate's revocation status. This process involves checking whether the CA's latest published CRL lists the certificate's serial number. Hierarchically, each CA in systems with multiple authorities manages its respective list. However, with indirect CRLs, one CA can assume responsibility for the revocation status of certificates issued by various authorities, centralizing this aspect in more complex PKI systems.
The format of a CRL is defined in the X.509 standard and in RFC 5280

Despite their critical role, CRLs face scalability challenges. As digital certificate issuance has increased, so has the size of these lists, leading to distribution and processing issues. These challenges have prompted adaptations such as Delta CRLs ($\Delta$ CRLs), which offer a condensed version of revocation updates, and Partitioned CRLs, which divide the list into smaller, more manageable segments.
CRL Distribution Points (CDPs), embedded within certificates, specify URLs for accessing the CRLs pertinent to each certificate. This innovation decentralizes distribution, allowing entities to access relevant revocation information directly. However, the main challenge with CRLs remains their delay in updating revocation information and the high bandwidth requirement for distributing extensive lists.

As decentralized systems like blockchain emerge, they present opportunities for transforming the CRL model. Such systems could distribute revocation information across a network, minimizing central CA reliance and potentially enhancing the efficiency and security of the revocation process in PKI systems.

\subsection{Online Certificate Status Protocol} 

The Online Certificate Status Protocol (OCSP) emerged as a solution in Public Key Infrastructure (PKI) for addressing the limitations in Certificate Revocation Lists (CRLs). OCSP facilitates real-time verification of digital certificate statuses, thereby resolving the delays associated with the CRL system. In OCSP's operational model, Certificate Authorities (CAs) maintain dedicated servers that actively respond to specific queries about a certificate's revocation status. This shift from the CRL's passive approach to an active query-response model significantly enhances the timeliness of certificate status verification.

In the OCSP framework, servers under CA management store the latest revocation information for each issued certificate. When a verifier, such as a user's web browser, needs to confirm a certificate's status, it actively queries the OCSP server. The server promptly responds with the current status, indicating whether the certificate is valid or revoked. This process ensures immediate access to revocation information, making OCSP essential in environments where certificate validity is critical. Various stakeholders engage in the OCSP process: CAs manage the OCSP servers, certificate holders (like domain owners) depend on these servers for their certificates' validity, and verifiers (users or their browsers) utilize this data for certificate validation. The CA's role is crucial as it updates the OCSP server with real-time revocation data, upon which verifiers rely for accurate certificate status.

Despite its advantages in real-time verification, OCSP introduces challenges such as increased communication between clients and servers, impacting network performance and user privacy. OCSP Stapling emerged to address these issues, where servers present a CA-provided, time-stamped OCSP response during the TLS handshake. This method reduces the demand on OCSP servers for individual verifications.
OCSP Must-Staple further secures online communications by ensuring browsers connect only to servers with a valid OCSP staple, preventing potential security risks from servers with revoked certificates.
Exploration into integrating OCSP within decentralized systems, like blockchain-based environments, is ongoing. Such integration could leverage OCSP's real-time verification while addressing the centralization challenges, presenting a promising direction for enhancing certificate revocation mechanisms in decentralized PKI systems.

The Public Key Infrastructure (PKI) has seen advancements by introducing various innovative approaches to certificate revocation. These methods have enhanced the traditional models of Certificate Revocation Lists (CRLs) and Online Certificate Status Protocol (OCSP), addressing their inherent limitations and adapting to the evolving digital security landscape.

Push-based revocation and the Authority Information Access (AIA) extension represent two advancements. Push-based revocation changes the dynamics of traditional revocation methods by enabling servers to inform clients about certificate status changes actively. This proactive approach ensures real-time updates and is ideal for environments requiring swift revocation information dissemination. AIA, on the other hand, adds a layer of efficiency in certificate verification by including crucial information for retrieving the issuing CA's certificate within X.509 certificates themselves.

Short-Term Certificate Revocation Lists (STCRLs) and the Automated Certificate Management Environment (ACME) are tailored to specific operational environments. STCRLs are particularly useful in contexts where certificates have shorter lifespans, enhancing distribution efficiency and updates. ACME automates the processes of certificate issuance, renewal, and revocation, benefiting automated environments like Let's Encrypt by reducing manual intervention and streamlining operations.

Certificate Transparency (CT) and different validity models, such as Short-Lived Certificates, offer solutions to persistent challenges in PKI systems. Certificate Transparency aids in detecting misused or unauthorized certificates through public, auditable logs, thereby enhancing the overall security of digital certificates. Short-lived certificates reduce the need for frequent revocation checks by having shorter validity periods, thus simplifying the overall management of digital certificates.

Assigning reason codes during revocation and managing cross-certificate revocation in complex PKI environments are crucial for maintaining transparency and trust in digital systems. Reason codes offer detailed explanations for revocations, such as compromise or affiliation changes, while cross-certificate revocation requires coordinated efforts to ensure the integrity of interconnected CAs.

In summary, revoking X.509 certificates in centralized systems is a critical function for maintaining the integrity and trustworthiness of digital communications. The evolution from CRLs to more sophisticated mechanisms like OCSP Stapling and Certificate Transparency reflects ongoing efforts to enhance certificate revocation processes' efficiency, reliability, and security.

\subsection{Complexities in Traditional PKI Systems}
The landscape of traditional Public Key Infrastructure extends beyond the realms of CRLs and OCSP. It encompasses various concepts such as Name Constraints, which dictate the scope of certificate applicability; the utilization of Short-Lived Certificates to reduce revocation needs; Proxy Certificates that delegate authorization; and Delegated Credentials for more flexible and secure certificate management. These components collectively enhance the adaptability and resilience of PKI systems in the governance of X.509 certificates.

% TODO: Add some revocation methods tailored for domains...Vanets, Manet

\begin{comment}

% Content:
The X.509 standard specifies a public key infrastructure and certificate format used in transport layer security (TLS), the basis for HTTPS~\cite{1189190}. HTTPS follows hierarchical structure where domain owner request X.509 certificates that authenticate them against users of their domain - websites. <add more description>. Once a domain owner proof ownership of a domain, a certificate authority can issue an x.509 certificate that technically bound a domain owners public key to the certificate.
Traditional PKI
Name Constraints
Short-Lived Certificates
Proxy Certificates
Delegated Credentials

TODO description TLS communication, signing certificates by CAs for domain owner..description of usage of x.509 for digital documents, id cards, pdf documents, diploma.. 

The X.509 standard also secures e-mail communication, and enables signing of digital documents. 
\end{comment}

\subsection{Transition to Decentralized Systems}
Outline the shift from centralized PKI systems to decentralized approaches, focusing on the limitations of traditional systems that prompted this transition. Introduce blockchain technology as a solution, emphasizing its potential in managing digital identities and credentials.

\section{Decentralized Credential Revocation}
Address the specific challenges faced in the revocation of verifiable credentials within decentralized systems. Discuss how blockchain technology and advanced cryptographic techniques like Zero-Knowledge Proofs (ZKPs) contribute to resolving these challenges.

\subsection{Comparative Analysis of Traditional and Decentralized Revocation Mechanisms}
Provide a critical comparison of traditional mechanisms (CRLs, OCSP) and decentralized approaches, highlighting the advantages and ongoing challenges in both realms.

\subsection{Prospects of Decentralized Systems in Overcoming PKI Limitations}
The advent of blockchain technology marks a significant milestone in the evolution of PKI systems. Blockchain's inherent characteristics of decentralization, immutability, and transparency offer a novel approach to managing digital certificates. In a blockchain-based PKI model, trust distribution across a network of nodes eliminates single points of failure inherent in centralized systems, thereby enhancing the overall resilience against security breaches.

\textbf{Decentralization and Enhanced Security. } Decentralized PKI systems leverage blockchain's distributed ledger technology to create a more secure and transparent mechanism for certificate management. By decentralizing the issuance and revocation of certificates, these systems reduce the reliance on central authorities and mitigate the risks associated with centralized control. The blockchain's cryptographic underpinnings further bolster these systems' security, ensuring the integrity of certificate data.

\textbf{User-Centric Control and Transparency. } A pivotal advantage of decentralized PKI is the empowerment of end-users with greater control over their digital identities and certificates. This user-centric approach aligns with Self-Sovereign Identity (SSI) principles, where individuals have direct ownership and control over their identity credentials. The transparent nature of blockchain allows for a more accessible and verifiable process of certificate validation and revocation, fostering trust among all participants in the digital ecosystem.

\begin{itemize}
    \item Historical Context of Credential Revocation: Start with a brief history of credential revocation mechanisms, tracing their evolution from the early days of Public Key Infrastructure (PKI) to the present.
    \item Evolution of credential revocation mechanisms: From traditional PKI to decentralized approaches.
    \item Brief history and evolution of credential revocation mechanisms, including traditional and decentralized approaches.
    \item Public Key Infrastructure (PKI): Explanation of PKI fundamentals relevant to credential management.
    \item Certificate Revocation Lists (CRLs): Exploration of the concept, operation, and limitations of CRLs.
    \item Online Certificate Status Protocol (OCSP): Discussion on OCSP, its role in real-time status verification, and its challenges.
    \item Transition to Decentralized Systems: Addressing the limitations of traditional systems and the emerging need for decentralized approaches, including a brief introduction to blockchain and its potential. Importance of credential revocation in the context of security and privacy in decentralized systems.
    \item Introduction to decentralized systems, providing a rationale for their emergence.
\end{itemize}

\begin{comment}
These issues motivate the general requirements for an
effective revocation strategy, which Larisch et al. [11] formally
enumerated as the following six criteria that a universal
revocation strategy should fulfill:
1) Efficiency - The revocation strategy should require
minimal network bandwidth, storage, and computational
resources.
2) Timeliness - Revocation status updates should be sent
frequently to ensure that they never become stale.
3) Failure Model - The strategy should enable clients to
adopt a hard-failure policy.
4) Privacy - The strategy should preserve client traffic
privacy.
5) Deployability - The revocation strategy should be
incrementally deployable and provide incentives for
adopters.
6) Auditability - Revocation information should be auditable
by other parties.

Incorporating a deeper analysis of the early and current revocation methods, along with their pros, cons, and potential adaptations in decentralized systems, is a robust approach for your SoK paper. In addition to describing each method, it’s important to maintain a high scientific level by including several key aspects:

Historical Evolution and Context: Provide a historical perspective on how and why specific revocation methods were developed. This should include the technological and security landscape at the time, giving context to the evolution of these methods.

Technical Details and Mechanisms: Offer a detailed technical explanation of each revocation method. This includes the underlying cryptographic principles, protocol specifics, and any relevant algorithms or models.

Performance Analysis: Analyze the performance of each revocation method in terms of efficiency, scalability, reliability, and response time. Use empirical data or simulations, if available, to support your analysis.

Security Implications: Discuss the security implications of each revocation method. This includes potential vulnerabilities, known attacks, and the overall impact on the security of the PKI system.

Comparative Analysis: Provide a comparative analysis of the methods, highlighting their strengths and weaknesses. This should be backed by evidence and research findings.

Adaptation in Decentralized Systems: Explore how these methods have been adapted or could be adapted in decentralized systems. Discuss the challenges and benefits of these adaptations.

Future Directions and Emerging Trends: Identify and discuss emerging trends in certificate revocation, such as new cryptographic techniques, AI/ML applications in revocation prediction, and the impact of quantum computing on certificate security.

Case Studies and Real-world Applications: Include case studies or real-world examples where different revocation methods have been implemented. Analyze their outcomes and lessons learned.

Standardization and Regulatory Considerations: Address any standardization efforts or regulatory considerations relevant to certificate revocation, including global and industry-specific compliance issues.

Expert Opinions and Industry Insights: Incorporate insights from industry experts, practitioners, and academicians. This can include quotes, interviews, or references to significant papers or reports.

By covering these areas, your SoK paper will provide a comprehensive, scientifically rigorous analysis of X.509 certificate revocation methods, their evolution, and their role in both traditional and decentralized PKI systems.



\end{comment}

% Backup Intro 28.3.24
\section{Introduction (1 page)}
\label{sec:introduction}
% TODO: go through all abbreviations, remove redundancy
% TODO: Rewrite Introduction according to change in scope from SoK to Taxonomy paper
Decentralized Credential Status Management (DCSM) represents a transformative shift in the landscape of digital trust, marking a departure from centralized Public Key Infrastructure (PKI) limitations. Blockchain technology and advanced cryptographic techniques, such as Zero-Knowledge Proofs (ZKP), Multi-Party Computation (MPC), and Fully Homomorphic Encryption (FHE), have paved the way for a new era in credential management. This paradigm shift addresses the systemic vulnerabilities, operational inefficiencies, and trust monopolies that plagued centralized PKI systems. By leveraging the inherent security, transparency, and immutability of distributed ledger technology, DCSM systems offer a promising solution to the challenges of centralized trust models. The evolution of PKI from the 1970s through the 2000s is characterized by the enhancement and standardization of centralized systems alongside decentralized models prioritizing user control and privacy. However, centralized PKI systems still need improvements and face challenges such as certificate chain validation and scenarios where revocation information is unavailable.

\textbf{Challenges. }
Centralized trust models in Public Key Infrastructure (PKI), especially those relying on X.509 certificates, confront significant challenges~\cite{10196098},~\cite{clark2013sok},~\cite{delignat2016cinderella}. Centralized architectures face security risks, particularly the vulnerability of CAs, requiring the revocation of compromised certificates~\cite{Berkowsky2017SecurityIW}. Certificate revocation was managed primarily through Certificate Revocation Lists (CRL) and remains a dominant methodology~\cite{10.1145/2815675.2815685}. However, revocation lists encountered scalability challenges due to the exponential increase in the volume of revoked certificates. To mitigate the constraints posed by CRLs, the Online Certificate Status Protocol (OCSP) evolved~\cite{santesson2013x}. Although the OCSP introduced real-time verification, it increased the communication overhead required for certificate status verification, imposing additional operational demands~\cite{munoz2002evaluation},~\cite{zhu2016measuring}. Despite the introduction of OCSP Must-Staple~\cite{chung2018web} and short-lived certificates~\cite{topalovic2012towards}, challenges such as irregular browser adoption still persist~\cite{8835212}. These challenges require reevaluating the management of the certificate status in the transition to decentralized systems~\cite{8406563}. The need to transition towards decentralized systems is emphasized by incidents of compromised CAs and issuance of fraudulent certificates, highlighting the vulnerability of centralized systems to security breaches. Durumeric et al.~\cite {durumeric2013analysis} analyze the HTTPS ecosystem and emphasize the fragility of centralized PKI, where a single point of failure can compromise web security globally. The switch from centralized to decentralized PKI systems marks a change in digital identity verification, addressing the limitations of centralized models~\cite{Fromknecht2014ADP},~\cite{Avellaneda2019DecentralizedIW}. Central to this change is blockchain technology, which introduces novel methodologies for managing identities and credentials~\cite{Lux2020DistributedLedgerbasedAW},~\cite{Sedlmeir2021DigitalIA}. 

\textbf{Contributions. }
This paper makes significant contributions to digital trust and credential management by introducing a comprehensive taxonomy that delineates the limitations inherent in centralized PKI, along with illuminating potential opportunities within decentralized PKI systems. Additionally, it presents a qualitative and empirical analysis that underpins the efficacy of decentralized mechanisms, notably those leveraging blockchain technology for credential status management. Furthermore, it proposes innovative methodologies that integrate advanced cryptographic techniques, enhancing the security and privacy of digital credentials, thus offering a novel perspective in the ongoing discourse on digital identity verification and management.

This paper distinguishes itself from existing research by providing a comprehensive and comparative analysis of traditional PKI components and methods alongside decentralized approaches. By offering a detailed overview of domain-specific requirements within decentralized environments for managing credential status, this work highlights the unique challenges and opportunities presented by DCSM systems. In doing so, it contributes to the ongoing discourse on the evolution of PKI from its centralized origins to the emerging decentralized alternatives, emphasizing the potential of DCSM in enhancing security, privacy, and efficiency in digital identity management. As the digital landscape continues to evolve, the insights and perspectives offered by this paper will serve as a foundation for future research and innovation in this critical area.
% Doing: shorten section II drastically. (2,5 - 3 pages max.)

==> working_folder/tablesBackup/2_comparison.tex <==
\begin{table*}[!htbp]
  \caption{Systematically assessment of Public Key Infrastructure (PKI) paradigms by juxtaposing centralized and decentralized schemas with operational attributes. The comparison highlights the pros and cons of each aspect. The comparison encapsulates the considerations relevant to adopting PKI systems, substantiated by various citations that facilitate an in-depth academic exploration.}
  \label{tab:comprehensive_PKI_evaluation}
  \centering
  \begin{tabularx}{\textwidth}{>{\hsize=0.8\hsize}X >{\hsize=1.1\hsize}X >{\hsize=1.1\hsize}X}
    \toprule
    \textbf{Aspect} & \centering{\textbf{Centralized PKI}} & \centering\arraybackslash{\textbf{Decentralized PKI}} \\
    \midrule
    Operational Efficiency & 
    \textit{Pros:} Efficient centralized management. \newline
    \textit{Cons:} Risk of centralized failures. [1]-[5] & 
    \textit{Pros:} Resilience against single points of failure. \newline
    \textit{Cons:} Complex setup and management. [6]-[10] \\
    \midrule
    Trust Model & 
    \textit{Pros:} Simplified identity validation through CAs. \newline
    \textit{Cons:} Potential for opaque trust decisions. [11]-[15] & 
    \textit{Pros:} Transparency in trust establishment. \newline
    \textit{Cons:} Delays due to distributed consensus. [16]-[20] \\
    \midrule
    Security & 
    \textit{Pros:} Centralized policy enforcement. \newline
    \textit{Cons:} High impact of breaches. [21]-[25] & 
    \textit{Pros:} Distributed nature mitigates targeted attacks. \newline
    \textit{Cons:} New security challenges. [26]-[30] \\
    \midrule
    Scalability & 
    \textit{Pros:} Scalable within a controlled growth. \newline
    \textit{Cons:} Limits in rapid scaling capabilities. [31]-[35] & 
    \textit{Pros:} Enhanced scalability through distributed systems. \newline
    \textit{Cons:} Performance issues at scale. [36]-[40] \\
    \midrule
    Privacy & 
    \textit{Pros:} Centralized data protection measures. \newline
    \textit{Cons:} Single point for potential data breaches. [41]-[45] & 
    \textit{Pros:} Improved privacy controls for users. \newline
    \textit{Cons:} Risks associated with ledger transparency. [46]-[50] \\
    \midrule
    Regulatory Adaptation & 
    \textit{Pros:} Established compliance pathways. \newline
    \textit{Cons:} Rigid in adapting to new regulations. [51]-[55] & 
    \textit{Pros:} Flexibility in regulatory innovation. \newline
    \textit{Cons:} Uncertainty in compliance standards. [56]-[60] \\
    \midrule
    Adaptation to Tech & 
    \textit{Pros:} Incremental technology integration. \newline
    \textit{Cons:} Slow adoption of breakthrough technologies. [61]-[65] & 
    \textit{Pros:} Quick to adopt and integrate new tech. \newline
    \textit{Cons:} Dependency on community consensus for updates. [66]-[70] \\
    \midrule
    Identity Management & 
    \textit{Pros:} Established identity verification processes. \newline
    \textit{Cons:} Limited control over personal data. [71]-[75] & 
    \textit{Pros:} Enables self-sovereign identity models. \newline
    \textit{Cons:} Challenges in achieving widespread acceptance. [76]-[80] \\
    \bottomrule
  \end{tabularx}
\end{table*}

==> working_folder/tablesBackup/2_summary.tex <==
\newcommand{\lowoverhead}{\ding{109}} % Empty circle
\newcommand{\moderateoverhead}{\ding{119}} % Half-filled circle
\newcommand{\highoverhead}{\ding{108}} % Filled circle

\begin{table*}[!htbp]
\caption{Comprehensive Historical Evolution of Public Key Infrastructure (PKI) with Enhanced Categories and Aspects}
\label{tab:comprehensive_pki_evolution}
\centering
\begin{tabular}{@{}p{1cm}p{0.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}@{}}
\toprule
\textbf{Milestone} & \textbf{Year} & \textbf{Key Contributions} & \textbf{Challenges} & \textbf{Impact on Digital Security} & \textbf{System Type} & \textbf{Algorithms} & \textbf{Attack Vectors} & \textbf{Applicability} & \textbf{Post Quantum Secure} \\
\midrule
Diffie-Hellman & 1976 & Introduced public key cryptography. & Distributing public keys securely. & Groundwork for secure communications. & Cryptographic Algorithm & Public key exchange & Man-in-the-middle & Both & \lowoverhead \\
RSA & 1978 & Secure data encryption and verification. & Key generation and encryption intensity. & Use of asymmetric cryptography. & Cryptographic Algorithm & Asymmetric encryption & Factorization & Both & \lowoverhead \\
X.509 & Late 1980s & Digital certificate format. & Complexity and interoperability. & Establishment of PKI. & Standard & -- & Impersonation, MiTM & Central & \lowoverhead \\
PGP & 1991 & Encryption control to individuals. & Public acceptance, legal challenges. & Email encryption and signatures. & Decentralized Trust Model & Symmetric, Asymmetric & Key distribution, Trust & Decentral & \moderateoverhead \\
SSL/TLS & Mid-1990s & Encryption standard for internet traffic. & Security vulnerabilities. & Secure web transactions. & Protocol & Symmetric, Asymmetric & Downgrade, MiTM & Central & \lowoverhead \\
Blockchain & 2008 & Trustless transactions model. & Scalability, energy consumption. & Digital trust and security concepts. & Decentralized System & Hash functions, PoW & 51\% attack, Sybil & Decentral & \moderateoverhead \\
Bitcoin & 2009 & Practical blockchain application. & Legal, regulatory acceptance. & Cryptocurrency development. & Cryptocurrency Implementation & SHA-256, PoW & 51\% attack, Wallet security & Decentral & \moderateoverhead \\
ACME & 2000s & Certificate issuance and renewal. & Automated process security. & Certificate lifecycle management. & Protocol & -- & Mis-issuance & Central & \highoverhead \\
Certificate Transparency & 2010s & Transparent certificate issuance. & Privacy, log integrity. & CA accountability and trust. & Security Enhancement & -- & Log poisoning & Central & \highoverhead \\
SSI & 2010s & Self-managed digital identities. & System adoption, interoperability. & User-centric identity models. & Identity Management System & DIDs, VCs & Identity theft & Decentral & \highoverhead \\
\bottomrule
\end{tabular}
\end{table*}
